SafetyPin: Encrypted Backups with Human-Memorable Secrets

We present the design and implementation of SafetyPin, a system for encrypted mobile-device backups. Like existing cloud-based mobile-backup systems, including those of Apple and Google, SafetyPin requires users to remember only a short PIN and defends against brute-force PIN-guessing attacks using hardware security protections. Unlike today's systems, SafetyPin splits trust over a cluster of hardware security modules (HSMs) in order to provide security guarantees that scale with the number of HSMs. In this way, SafetyPin protects backed-up user data even against an attacker that can adaptively compromise many of the system's constituent HSMs. SafetyPin provides this protection without sacrificing scalability or fault tolerance. Decentralizing trust while respecting the resource limits of today's HSMs requires a synthesis of systems-design principles and cryptographic tools. We evaluate SafetyPin on a cluster of 100 low-cost HSMs and show that a SafetyPin-protected recovery takes 1.01 seconds. To process 1B recoveries a year, we estimate that a SafetyPin deployment would need 3,100 low-cost HSMs.

==> figs/colors.tex <==
\definecolor{few-gray-bright}{HTML}{010202}
\definecolor{few-red-bright}{HTML}{EE2E2F}
\definecolor{few-green-bright}{HTML}{008C48}
\definecolor{few-blue-bright}{HTML}{185AA9}
\definecolor{few-orange-bright}{HTML}{F47D23}
\definecolor{few-purple-bright}{HTML}{662C91}
\definecolor{few-brown-bright}{HTML}{A21D21}
\definecolor{few-pink-bright}{HTML}{B43894}
\definecolor{few-gray}{HTML}{737373}
\definecolor{few-red}{HTML}{F15A60}
\definecolor{few-green}{HTML}{7AC36A}
\definecolor{few-blue}{HTML}{5A9BD4}
\definecolor{few-orange}{HTML}{FAA75B}
\definecolor{few-purple}{HTML}{9E67AB}
\definecolor{few-brown}{HTML}{CE7058}
\definecolor{few-pink}{HTML}{D77FB4}
\definecolor{few-gray-light}{HTML}{CCCCCC}
\definecolor{few-red-light}{HTML}{F2AFAD}
\definecolor{few-green-light}{HTML}{D9E4AA}
\definecolor{few-blue-light}{HTML}{B8D2EC}
\definecolor{few-orange-light}{HTML}{F3D1B0}
\definecolor{few-purple-light}{HTML}{D5B2D4}
\definecolor{few-brown-light}{HTML}{DDB9A9}
\definecolor{few-pink-light}{HTML}{EBC0DA}


==> figs/cost2.tex <==
\begin{table}
\centering
{\small
\begin{tabular}[t]{l|rcr|r}
\toprule
%&\multicolumn{2}{c}{\textbf{HSMs}}  
  &\multicolumn{1}{c}{\textbf{HSM Qty.}} &\multicolumn{1}{c}{$\fevil$} &\multicolumn{1}{c|}{$N_\mathsf{evil}$}
  &\multicolumn{1}{c}{\textbf{Cost}} \\
  \midrule
  SoloKey~\cite{solokeys} &  3,037 & $1/16$ & 189 & \$60.7K \\
  YubiHSM2~\cite{yubico-hsm} &  1,732 & $1/16$ & 108 & \$1.1M \\
  SafeNet A700~\cite{safenet}&  40 & $1/20$ & 2& \$738.7K \\
  -- 10 evil HSMs & 320 & $1/32$ & 10 &\$3.0M \\
  -- 50 evil HSMs & 800 & $1/16$ & 50 & \$14.8M \\ \midrule
%Baseline & 5 & 0 & \$92.3K \\\midrule
\multicolumn{4}{l}{\emph{Estimated cost of storing 4GB $\times$ $10^9$ users per year:}} & \$600M \\
\bottomrule
\end{tabular}
}
  \caption[]{The estimated hardware cost of a \name deployment supporting
one billion users, if each user recovers once per year.
  The $N_\textsf{evil}$ number is how many corrupt
  HSMs the deployment tolerates.\par
\smallskip
{\footnotesize {\setstretch{0.8}
We estimate the storage cost using
AWS S3 infrequent access~\cite{s3}
(\$0.0125 per GB/month). 
We estimate YubiHSM2 and SafeNet HSM throughput using
their data sheets (Table~\ref{tab:hsm}). 
When computing the number of HSMs necessary
to service a billion users, we account for 
key-rotation time. 
A cluster of 40 SafeNet HSMs can meet the
throughput demands of one billion users, so
we also consider larger deployments tolerating
more compromised HSMs. 
\par }}}
\label{tab:e2e-cost}
\end{table}
% glacier tier $.004/GB


==> figs/tab-cost.tex <==
\begin{table}[ht]
\centering 
{\footnotesize
\begin{tabular}[t]{lrrr}
\toprule
    \textbf{Item} & \textbf{Number} & \textbf{Cost/item} & \textbf{Subtotal} \\
\midrule
    SoloKey~\cite{solokeys} & 100 & \$20.00 & \$2,000.00  \\  
    Anker USB hub~\cite{usbhub} & 10 & \$52.99 & \$529.90 \\
    USB PCIe card~\cite{pcie-cards} & 2 & \$159.00 & \$316.00 \\
    USB cable~\cite{cables} & 10 & \$5.98 & \$59.80 \\
\midrule
    Grand total & & & \$2,905.70 \\
\bottomrule 
\end{tabular}
}
\caption{Retail cost of our experimental HSM cluster.} 
\label{tab:cost}
\end{table}


==> fonts.tex <==

\usepackage[T1]{fontenc}
\usepackage{newtxmath}
\usepackage{newtxtext}

% Use slightly smaller-than-default \texttt
\usepackage[scaled=.8]{beramono}

% Use normal mathcal
\DeclareMathAlphabet\mathcal{OMS}{cmsy}{m}{n}
\SetMathAlphabet\mathcal{bold}{OMS}{cmsy}{b}{n}

% Use normal mathsf
\SetMathAlphabet{\mathsf}{normal}{OT1}{cmss}{m}{n}
\SetMathAlphabet{\mathsf}{bold}{OT1}{cmss}{bx}{n}

% Use AMS mathbb
\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareSymbolFontAlphabet{\mathbb}{AMSb}


% Use times for numbers
\DeclareSymbolFont{numbers}{T1}{ptm}{m}{n}
\SetSymbolFont{numbers}{bold}{T1}{ptm}{bx}{n}
\DeclareMathSymbol{0}\mathalpha{numbers}{"30}
\DeclareMathSymbol{1}\mathalpha{numbers}{"31}
\DeclareMathSymbol{2}\mathalpha{numbers}{"32}
\DeclareMathSymbol{3}\mathalpha{numbers}{"33}
\DeclareMathSymbol{4}\mathalpha{numbers}{"34}
\DeclareMathSymbol{5}\mathalpha{numbers}{"35}
\DeclareMathSymbol{6}\mathalpha{numbers}{"36}
\DeclareMathSymbol{7}\mathalpha{numbers}{"37}
\DeclareMathSymbol{8}\mathalpha{numbers}{"38}
\DeclareMathSymbol{9}\mathalpha{numbers}{"39}

% Use times for operators
\SetSymbolFont{numbers}{bold}{T1}{ptm}{b}{n}
\makeatletter
\renewcommand{\operator@font}{\mathgroup\symnumbers}
\makeatother

% 10pt on 11pt
\makeatletter
\iffalse
\renewcommand\normalsize{%
   \@setfontsize\normalsize{10pt}{11.55pt}%
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}

\renewcommand\small{%
  \@setfontsize\small{9pt}{2pt}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\makeatother
\fi


